Inclusive Electron Scattering From Nuclei at x>1 and High Q^2

CEBAF experiment e89-008 measured inclusive electron scattering from nuclei in a Q^2 range between 0.8 and 7.3 (GeV/c)^2 for x_{Bjorken} \gtorder 1. The cross sections for scattering from D, C, Fe, and Au were measured. The C, Fe, and Au data have been analyzed in terms of F(y) to examine $y$-scaling of the quasielastic scattering, and to study the momentum distribution of the nucleons in the nucleus. The data have also been analyzed in terms of the structure function \nu W_2 to examine scaling of the inelastic scattering in x and \xi, and to study the momentum distribution of the quarks. In the regions where quasielastic scattering dominates the cross section (low Q^2 or large negative values of y), the data are shown to exhibit y-scaling. However, the y-scaling breaks down once the inelastic contributions become large. The data do not exhibit x-scaling, except at the lowest values of x, while the structure function does appear to scale in the Nachtmann variable, \xi.

==> data_tables.tex <==
This section contains the cross sections (corrected for all inefficiencies
and radiatively unfolded) for the Carbon, Iron, and Gold data as a function
of scattering angle.  All data was taken at a beam energy of 4.045 GeV.  In
addition to the energy loss and cross section, $y$, the quasielastic
scaling function $F(y)$, $x$,$\xi$, and the structure function per nucleon
$\nu W_2 /A$ are included.  $d\sigma 1$ is the statistical uncertainty for the
cross section, $F(y)$, and $\nu W_2$. $d\sigma 2$ is the systematic
uncertainty (as discussed in section \ref{sec_syserr}). The systematic
uncertainty includes everything except the uncertainty in $R=\sigma_L /
\sigma_T$ (discussed in section \ref{sec_structurefunc}).  All of the HMS data
is included, along with the SOS data at 74$\deg$.  The SOS data taken at
30$\deg$ and 55$\deg$ was compared to the HMS data in order to determine
the SOS normalization (see section\ref{sec_sosnorm}).  Final-state interactions
are expected to be largest at very low energy loss \cite{day_review}, and
so only points with energy loss more than 100 MeV above the elastic peak are
included ($\nu - \nu_{elas} >$ 100 MeV).

{\tiny

\input{data/c_15.table} \clearpage
\input{data/fe15.table} \clearpage
\input{data/au15.table} \clearpage
\input{data/c_23.table} \clearpage
\input{data/fe23.table} \clearpage
\input{data/au23.table} \clearpage
\input{data/c_30.table} \clearpage
\input{data/fe30.table} \clearpage
\input{data/au30.table} \clearpage
\input{data/c_37.table} \clearpage
\input{data/fe37.table} \clearpage
% \input{data/au37.table} \clearpage	!all Au 37 degree data cut (DC problems).
\input{data/c_45.table} \clearpage
\input{data/fe45.table} \clearpage
\input{data/au45.table} \clearpage
\input{data/c_55.table} \clearpage
\input{data/fe55.table} \clearpage
\input{data/au55.table} \clearpage
\input{data/c_74s.table} \clearpage
\input{data/fe74s.table} \clearpage
\input{data/au74s.table} \clearpage}


==> equation.tex <==
\begin{equation}
x=y
\label{temp}
\end{equation}

